Real-Time Panoptic Segmentation from Dense Detections

Panoptic segmentation is a complex full scene parsing task requiring simultaneous instance and semantic segmentation at high resolution. Current state-of-the-art approaches cannot run in real-time, and simplifying these architectures to improve efficiency severely degrades their accuracy. In this paper, we propose a new single-shot panoptic segmentation network that leverages dense detections and a global self-attention mechanism to operate in real-time with performance approaching the state of the art. We introduce a novel parameter-free mask construction method that substantially reduces computational complexity by efficiently reusing information from the object detection and semantic segmentation sub-tasks. The resulting network has a simple data flow that does not require feature map re-sampling or clustering post-processing, enabling significant hardware acceleration. Our experiments on the Cityscapes and COCO benchmarks show that our network works at 30 FPS on 1024x2048 resolution, trading a 3% relative performance degradation from the current state of the art for up to 440% faster inference.

==> figures/property-example.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.4\linewidth}
        \includegraphics[width=0.95\linewidth]{figures/source/example1_crop.png}
        \caption{}
        \label{fig:box-compensation}
    \end{subfigure}%
    \begin{subfigure}[b]{0.6\linewidth}
        \includegraphics[width=0.95\linewidth]{figures/source/example2_crop.png}
        \caption{}
        \label{fig:occlusion}
    \end{subfigure}
\caption{\textbf{Challenging Mask Reconstruction} Case (a) gives an example of our accurate mask reconstruction even when the proposal bounding box (with highest confidence) is not accurate. Case (b) provide a typical example where our algorithm is very good at handling occlusions in objects. }
\label{fig:property}
\end{figure}

==> sup_tables/levelness.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c}
\toprule
% Method & 
Levelness & PQ & $\text{PQ}^{th}$ & $\text{PQ}^{st}$ & mIoU & AP & Inference Time \\ \hline
\checkmark  & 55.5 & 47.6 & 61.2 & 74.7 & 26.7 & 77ms\\ \hline
$\times$ & 56.7 & 48.0 & 62.9 & 75.1 & 26.9 & 83ms\\ \hline
\hline
\end{tabular}%
}
\caption{\textbf{Performance of Our Proposed Framework with or without Levelness}}
\label{tab:wo_levelness}
\end{table}

==> tables/coco_performance_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[t]
\centering
% \resizebox{\linewidth}{!}{%
\resizebox{0.85\width}{!}{%
\begin{tabular}{c|c|c|cc|cc|cc}

Method & Backbone & PQ & \multicolumn{1}{c|}{$\text{PQ}^{th}$} & $\text{PQ}^{st}$ & \multicolumn{1}{c|}{mIoU} & \multicolumn{1}{c|}{AP} & \multicolumn{1}{c|}{GPU} & \multicolumn{1}{c}{Inference Time}\\ \hline
\multicolumn{9}{c}{\textbf{Two-Stage}} \\ \hline
%
AUNet~\cite{li2019attention} & ResNet-50-FPN & 39.6  & 49.1 & 25.2 & 45.1 & \multicolumn{1}{c|}{34.7} & \\ \hline
%
UPSNet~\cite{xiong2019upsnet} & ResNet-50-FPN & 42.5  & 48.5 & 33.4 & 54.3 & \multicolumn{1}{c|}{34.3} & \\ \hline
%
\multicolumn{9}{c}{\textbf{Single-Stage}}\\\hline
%
DeeperLab~\cite{deeperlab2019} & Xception-71 & 33.8 & - & - & - & \multicolumn{1}{c|}{-} & v100 & 94ms \\ \hline
%
SSAP~\cite{gao2019ssap} &  ResNet-50  & 36.5 & - & - & - & \multicolumn{1}{c|}{-} & - & - \\ \hline
%
Ours & ResNet-50-FPN & \textbf{37.1} & \textbf{41.0} & \textbf{31.3}  &\textbf{53.2}& \multicolumn{1}{c|}{\textbf{21.6}} & v100 & 76ms \\ \hline
\end{tabular}%
}
\caption{Performance-COCO-val}
\label{tab:pq-coco}
\end{table*}
\vspace{-3mm}

==> tables/inference-time-table-python-coco.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lllll}
\multicolumn{1}{l|}{Method} & \multicolumn{1}{l|}{Backbone} & \multicolumn{1}{l|}{GPU} & \multicolumn{1}{l|}{PQ} & \multicolumn{1}{l}{Inference Time } \\ \hline
% \multicolumn{1}{l|}{DeeperLab} & \multicolumn{1}{l|}{Wider MNV2} & \multicolumn{1}{l|}{V100} & \multicolumn{1}{l|}{27.9} & \multicolumn{1}{l}{58ms} \\ \hline
\multicolumn{1}{l|}{DeeperLab} & \multicolumn{1}{l|}{Xception-71} & \multicolumn{1}{l|}{V100} & \multicolumn{1}{l|}{33.8} & \multicolumn{1}{l}{94ms} \\ \hline
\multicolumn{1}{l|}{Ours} & \multicolumn{1}{l|}{R-50-FPN} & \multicolumn{1}{l|}{V100} & \multicolumn{1}{l|} {36.9}& \multicolumn{1}{l}{76ms} \\ \hline
% additional hline seperating different test GPU
\vspace{-10pt}
\\\hline
\multicolumn{1}{l|}{Ours} & \multicolumn{1}{l|}{?} & \multicolumn{1}{l|}{V100} & \multicolumn{1}{l|}{?} & \multicolumn{1}{l}{?} \\ \hline

\end{tabular}%
}
\caption{Inference time on COCO-Val Set. Pytorch, full resolution.}
\label{tab:inference-cityscapes}
\end{table}

==> tables/inference-time-table-pytorch.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lllll}
\hline
\multicolumn{1}{l|}{Method} & \multicolumn{1}{l|}{Backbone} & \multicolumn{1}{l|}{GPU} & \multicolumn{1}{l|}{PQ} & \multicolumn{1}{l}{Inference Time} \\ \hline
\multicolumn{1}{l|}{DeeperLab} & \multicolumn{1}{l|}{LW-MNV2} & \multicolumn{1}{l|}{V100} & \multicolumn{1}{l|}{48.1} & \multicolumn{1}{l}{251ms} \\ \hline
\multicolumn{1}{l|}{DeeperLab} & \multicolumn{1}{l|}{Xcep-71} & \multicolumn{1}{l|}{V100} & \multicolumn{1}{l|}{56.5} & \multicolumn{1}{l}{312ms} \\ \hline
\multicolumn{1}{l|}{SSAP} & \multicolumn{1}{l|}{R-50} & \multicolumn{1}{l|}{TitanX 1080Ti} & \multicolumn{1}{l|}{56.6} & \multicolumn{1}{l}{$>$260ms} \\ \hline
\hline
\multicolumn{1}{l|}{Ours-R-18} & \multicolumn{1}{l|}{R-18-FPN} & \multicolumn{1}{l|}{V100} & \multicolumn{1}{l|}{55.5} & \multicolumn{1}{l}{77ms} \\ \hline
\multicolumn{1}{l|}{Ours-R-34} & \multicolumn{1}{l|}{R-34-FPN} & \multicolumn{1}{l|}{V100} & \multicolumn{1}{l|}{56.8} & \multicolumn{1}{l}{83ms} \\ \hline
\multicolumn{1}{l|}{Ours} & \multicolumn{1}{l|}{R-50-FPN} & \multicolumn{1}{l|}{V100} & \multicolumn{1}{l|}{58.3} & \multicolumn{1}{l}{99ms} \\ \hline
% additional hline seperating different test GPU
\vspace{-10pt}
% \\\hline
% \multicolumn{1}{l|}{FPSNet} & \multicolumn{1}{l|}{R-50-FPN} & \multicolumn{1}{l|}{TITAN RTX} & \multicolumn{1}{l|}{55.1} & \multicolumn{1}{l}{114} \\ \hline
% \multicolumn{1}{l|}{Ours-R-18} & \multicolumn{1}{l|}{R-18-FPN} & \multicolumn{1}{l|}{TITAN RTX} & \multicolumn{1}{l|}{?} & \multicolumn{1}{l}{?} \\ \hline
% \multicolumn{1}{l|}{Ours-R-34} & \multicolumn{1}{l|}{R-34-FPN} & \multicolumn{1}{l|}{TITAN RTX} & \multicolumn{1}{l|}{?} & \multicolumn{1}{l}{?} \\ \hline
% \multicolumn{1}{l|}{Ours} & \multicolumn{1}{l|}{R-50-FPN} & \multicolumn{1}{l|}{TITAN RTX} & \multicolumn{1}{l|}{?} & \multicolumn{1}{l}{?} \\ \hline
\end{tabular}%
}
\caption{Inference time on Cityscapes-Val Set. Pytorch, full resolution.}
\label{tab:inference-coco}
\end{table}

==> tables/performance-cityscapes-val.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|c|c|cc|cc}

Method & Backbone & \multicolumn{1}{c|}{PQ}  & \multicolumn{1}{c|}{PQth} & PQst & \multicolumn{1}{c|}{mIoU} & \multicolumn{1}{c}{AP} \\ \hline
\multicolumn{7}{c}{\textbf{Two-Stage}} \\ \hline
% DeeperLab~\cite{deeperlab2019} &  &  &  &  &  &  &  & \multicolumn{1}{c}{} \\ \hline
% DeeperLab~\cite{deeperlab2019} &  &  &  &  &  &  &  & \multicolumn{1}{c}{} \\ \hline
TASCNet~\cite{li2018learning} &R50-FPN  & 55.9 &  50.5& 59.8 & - & \multicolumn{1}{c}{-} \\ \hline
AUNet\cite{li2019attention} & R50-FPN&56.4  &  52.7& 59.0 & 73.6& \multicolumn{1}{c}{33.6} \\ \hline
Panoptic-FPN~\cite{kirillov2019panoptic2} & R50-FPN& 57.7 & 51.6& 62.2  &  77.8& \multicolumn{1}{c}{37.6} \\ \hline
UPSNet~\cite{xiong2019upsnet} & R50-FPN & 59.3 & 62.7 & 54.6 & 75.2 &   \multicolumn{1}{c}{33.3} \\ \hline
Seamless~\cite{porzi2019seamless} & R50-FPN & 59.8 & 63.6 & 54.6 &  76.2& \multicolumn{1}{c}{33.0} \\ \hline
Seamless~\cite{porzi2019seamless}-freeBN & R50-FPN & 60.2 & 63.6 & 55.6 &  74.9& \multicolumn{1}{c}{33.3} \\ \hline
% \hline  % hline for singleshot methods
\multicolumn{7}{c}{\textbf{Single-Stage}} \\ \hline
SSAP~\cite{gao2019ssap} & R50 & 56.6 & 49.2 & - & - & \multicolumn{1}{c}{31.5} \\ \hline
FPSNet~\cite{de2019fast} & R50-FPN & 55.1 & 48.3 & 60.1 & - & \multicolumn{1}{c}{-} \\ \hline
DeeperLab~\cite{deeperlab2019} & Xcep-71 & 56.5 & - & - & - & \multicolumn{1}{c}{-} \\ \hline
% source:a7n1yk62
Ours & R50-FPN  & \textbf{58.8} &\textbf{51.6}  & \textbf{63.7}& \textbf{76.8} & \multicolumn{1}{c}{\textbf{31.0}} \\ \hline
\hline
\end{tabular}%
}
\caption{Performance-cityscapes-val
}
\label{tab:pq-cityscapes}
\end{table}


% Let's add PQ+ to the paper here:

==> tables/performance-coco-val.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|c|c|cc|cc}

Method & Backbone & \multicolumn{1}{c|}{PQ} & \multicolumn{1}{c|}{PQth} & PQst & \multicolumn{1}{c}{mIoU} & \multicolumn{1}{c}{AP} \\ \hline
\multicolumn{7}{c}{\textbf{Two-Stage}}\\\hline
AUNet~\cite{li2019attention} &  R50-FPN& 39.6  & 49.1 & 25.2 & 45.1 & \multicolumn{1}{c}{34.7} \\ \hline
UPSNet~\cite{xiong2019upsnet} &  R50-FPN& 42.5  & 48.5 & 33.4 & 54.3 & \multicolumn{1}{c}{34.3} \\ \hline
\multicolumn{7}{c}{\textbf{Single-Stage}}\\\hline
DeeperLab~\cite{deeperlab2019} & Xcep-71 & 33.79 & - & - & - & \multicolumn{1}{c}{-} \\ \hline

Ours &  R50-FPN& \textbf{36.9}  &\textbf{41.2} & \textbf{30.6}  &\textbf{52.8}& \multicolumn{1}{c}{\textbf{21.8}} \\ \hline
\end{tabular}%
}
\caption{Performance-COCO-val
}
\label{tab:pq-coco}
\end{table}

==> tables/tensorRT.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lllll}

\end{tabular}%
}
\caption{Inference time on Cityscapes-Val Set. Pytorch, full resolution.}
\label{tab:inference-coco}
\end{table}
